Synthetic Photography Detection: A Visual Guidance for Identifying Synthetic Images Created by AI

Artificial Intelligence (AI) tools have become incredibly powerful in generating synthetic images. Of particular concern are generated images that resemble photographs as they aspire to represent real world events. Synthetic photographs may be used maliciously by a broad range of threat actors, from scammers to nation-state actors, to deceive, defraud, and mislead people. Mitigating this threat usually involves answering a basic analytic question: Is the photograph real or synthetic? To address this, we have examined the capabilities of recent generative diffusion models and have focused on their flaws: visible artifacts in generated images which reveal their synthetic origin to the trained eye. We categorize these artifacts, provide examples, discuss the challenges in detecting them, suggest practical applications of our work, and outline future research directions.

==> figures/peope_eyes_and_teeth.tex <==

\begin{figure}[h]
\centering

  \imagewithcropbelow{images/humans/linkedin/SD15_realisticVision_linkedin_1.png}{0.3}{0.5}{0.7}{0.7}{0.2\textwidth}{}
  \quad

    \imagewithcropbelow{images/humans/linkedin/SD15_realisticVision_linkedin_2.png}{0.35}{0.725}{0.6}{0.85}{0.2\textwidth}{}
     \quad

  \imagewithcropbelow{images/humans/linkedin/sdxl_juggernaut_xl_v8_linkedin_4.png}{0.325}{0.675}{0.575}{0.8}{0.2\textwidth}{}
 \quad

    \imagewithcropbelow{images/humans/linkedin/real_portrait_cropped_1.jpg}{0.3}{0.48}{0.68}{0.67}{0.2\textwidth}{Real}
    \quad

  \imagewithcropbelow{images/humans/linkedin/sdxl_juggernaut_xl_v8_8.png}{0.4}{0.55}{0.5}{0.617}{0.2\textwidth}{}
  \quad

    \imagewithcropbelow{images/humans/linkedin/sdxl_juggernaut_xl_v8_9.png}{0.4}{0.55}{0.55}{0.651}{0.2\textwidth}{}
    \quad

    \imagewithcropbelow{images/humans/linkedin/sdxl_juggernaut_xl_v8_10.png}{0.45}{0.525}{0.575}{0.61}{0.2\textwidth}{}
    \quad

    \imagewithcropbelow{images/humans/linkedin/real_portrait_cropped_1.jpg}{0.33}{0.25}{0.59}{0.43}{0.2\textwidth}{Real}

  \caption{Eye artifacts can best be found by zooming in very closely on the image. The picture at the right shows a real photograph as a comparison (Source: Philip White on \href{https://unsplash.com/photos/a-woman-standing-in-front-of-a-sculpture-O3D-teBz0Bg}{Unsplash}). It shows that a certain asymmetry occurs naturally with eyes and does not necessarily indicate that the image has been generated. On the other hand, it is extremely rare for irises and pupils in real people not to be round or to have outlines that look somehow "jagged " or “frayed” (TODO: we have a paper source for this statement, add citation?).}

  \label{fig:people:eyes_teeth}
\end{figure}

